Planning Not to Talk: Multiagent Systems that are Robust to Communication Loss

In a cooperative multiagent system, a collection of agents executes a joint policy in order to achieve some common objective. The successful deployment of such systems hinges on the availability of reliable inter-agent communication. However, many sources of potential disruption to communication exist in practice, such as radio interference, hardware failure, and adversarial attacks. In this work, we develop joint policies for cooperative multiagent systems that are robust to potential losses in communication. More specifically, we develop joint policies for cooperative Markov games with reach-avoid objectives. First, we propose an algorithm for the decentralized execution of joint policies during periods of communication loss. Next, we use the total correlation of the state-action process induced by a joint policy as a measure of the intrinsic dependencies between the agents. We then use this measure to lower-bound the performance of a joint policy when communication is lost. Finally, we present an algorithm that maximizes a proxy to this lower bound in order to synthesize minimum-dependency joint policies that are robust to communication loss. Numerical experiments show that the proposed minimum-dependency policies require minimal coordination between the agents while incurring little to no loss in performance; the total correlation value of the synthesized policy is one fifth of the total correlation value of the baseline policy which does not take potential communication losses into account. As a result, the performance of the minimum-dependency policies remains consistently high regardless of whether or not communication is available. By contrast, the performance of the baseline policy decreases by twenty percent when communication is lost.

==> tikz/success_prob_vs_iters_aux_action.tex <==
% This file was created with tikzplotlib v0.9.12.
% \begin{tikzpicture}

% \begin{axis}[
% legend cell align={left},
% legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   at={(0.03,0.03)},
%   anchor=south west,
%   draw=white!80!black
% },
% tick align=outside,
% tick pos=left,
% title={Policy Success Probability During Synthesis},
% x grid style={white!69.0196078431373!black},
% xlabel={Number of Convex-Concave Iterations},
% xmajorgrids,
% xmin=-4.95, xmax=103.95,
% xtick style={color=black},
% y grid style={white!69.0196078431373!black},
% ylabel={Total Correlation Value},
% ymajorgrids,
% ymin=-0.732259762120947, ymax=1.0810631565931,
% ytick style={color=black}
% ]
\addplot [ultra thick, blue, mark=*, mark size=0, mark options={solid}]
table {%
0 0.347267771313956
1 0.363633197625958
2 0.409598840745856
3 0.483198494230437
4 0.578928106924863
5 0.683391740840553
6 0.777726069955075
7 0.848361527968071
8 0.893942130126948
9 0.920795451268541
10 0.935926651788902
11 0.944387259575197
12 0.949430412814631
13 0.952988974819143
14 0.955726067726352
15 0.957474941527844
16 0.958362914286858
17 0.95882847119927
18 0.959139475296815
19 0.959385769601055
20 0.959593781542775
21 0.959764693582641
22 0.959909572010445
23 0.960051540175686
24 0.960188981101009
25 0.960310071900513
26 0.960412182503393
27 0.960510455811873
28 0.960618511802193
29 0.960734915567934
30 0.960854069164287
31 0.960972640884844
32 0.961089280157399
33 0.961203499829196
34 0.961314956856813
35 0.961423934150375
36 0.961530026076308
37 0.961633045040178
38 0.96173264101209
39 0.96182887200955
40 0.961921023907814
41 0.962008723566031
42 0.96209157954503
43 0.962169198812907
44 0.962241066207193
45 0.962307526251855
46 0.962368431485765
47 0.962424332547116
48 0.962474977243686
49 0.962521314890252
50 0.962562051655844
51 0.96259511715179
52 0.962614909989117
53 0.962626233635301
54 0.962647478504148
55 0.962680694539066
56 0.962719162448406
57 0.962757758098293
58 0.962796100536428
59 0.962834314143912
60 0.962871616634544
61 0.962908160045604
62 0.962944093768858
63 0.962979480568292
64 0.963014391638547
65 0.963048622223279
66 0.96308271894436
67 0.963116250278014
68 0.963149312842644
69 0.963181823636873
70 0.963213781446946
71 0.963244925250154
72 0.963275787809858
73 0.963306012801431
74 0.963335358654892
75 0.963364373729731
76 0.963392706817051
77 0.963420345084945
78 0.963447017020388
79 0.96347340796086
80 0.963499008628701
81 0.963523831617543
82 0.96354770610279
83 0.963571117522508
84 0.963593651164945
85 0.96361531429065
86 0.963636168845043
87 0.963655875265154
88 0.963674992800273
89 0.963692694683515
90 0.963709883173988
91 0.963725907516986
92 0.963740713103283
93 0.963754298952595
94 0.963766599533411
95 0.963777533619192
96 0.963787056067577
97 0.963795037199582
98 0.963801444830457
99 0.963806173147503
};
\addlegendentry{\(\policy_{MD}\), Full Comm.}

\addplot [ultra thick, blue, dashed]
table {%
0 0.156
1 0.185
2 0.189
3 0.239
4 0.33
5 0.382
6 0.484
7 0.517
8 0.524
9 0.58
10 0.624
11 0.641
12 0.682
13 0.761
14 0.851
15 0.884
16 0.919
17 0.934
18 0.945
19 0.937
20 0.946
21 0.935
22 0.951
23 0.958
24 0.94
25 0.947
26 0.942
27 0.947
28 0.946
29 0.964
30 0.95
31 0.946
32 0.957
33 0.948
34 0.949
35 0.955
36 0.952
37 0.949
38 0.95
39 0.958
40 0.957
41 0.952
42 0.963
43 0.947
44 0.95
45 0.954
46 0.953
47 0.958
48 0.96
49 0.978
50 0.959
51 0.968
52 0.952
53 0.972
54 0.95
55 0.966
56 0.954
57 0.959
58 0.968
59 0.962
60 0.967
61 0.957
62 0.952
63 0.97
64 0.95
65 0.966
66 0.956
67 0.962
68 0.957
69 0.966
70 0.96
71 0.96
72 0.968
73 0.958
74 0.952
75 0.964
76 0.973
77 0.966
78 0.967
79 0.968
80 0.973
81 0.96
82 0.95
83 0.96
84 0.952
85 0.96
86 0.962
87 0.956
88 0.948
89 0.964
90 0.961
91 0.953
92 0.962
93 0.953
94 0.966
95 0.965
96 0.957
97 0.964
98 0.966
99 0.956
};
\addlegendentry{\(\policy_{MD}\), No Comm.}

\addplot [ultra thick, red, mark=*, mark size=0, mark options={solid}]
table {%
0 0.998639387560641
1 0.998639387560641
2 0.998639387560641
3 0.998639387560641
4 0.998639387560641
5 0.998639387560641
6 0.998639387560641
7 0.998639387560641
8 0.998639387560641
9 0.998639387560641
10 0.998639387560641
11 0.998639387560641
12 0.998639387560641
13 0.998639387560641
14 0.998639387560641
15 0.998639387560641
16 0.998639387560641
17 0.998639387560641
18 0.998639387560641
19 0.998639387560641
20 0.998639387560641
21 0.998639387560641
22 0.998639387560641
23 0.998639387560641
24 0.998639387560641
25 0.998639387560641
26 0.998639387560641
27 0.998639387560641
28 0.998639387560641
29 0.998639387560641
30 0.998639387560641
31 0.998639387560641
32 0.998639387560641
33 0.998639387560641
34 0.998639387560641
35 0.998639387560641
36 0.998639387560641
37 0.998639387560641
38 0.998639387560641
39 0.998639387560641
40 0.998639387560641
41 0.998639387560641
42 0.998639387560641
43 0.998639387560641
44 0.998639387560641
45 0.998639387560641
46 0.998639387560641
47 0.998639387560641
48 0.998639387560641
49 0.998639387560641
50 0.998639387560641
51 0.998639387560641
52 0.998639387560641
53 0.998639387560641
54 0.998639387560641
55 0.998639387560641
56 0.998639387560641
57 0.998639387560641
58 0.998639387560641
59 0.998639387560641
60 0.998639387560641
61 0.998639387560641
62 0.998639387560641
63 0.998639387560641
64 0.998639387560641
65 0.998639387560641
66 0.998639387560641
67 0.998639387560641
68 0.998639387560641
69 0.998639387560641
70 0.998639387560641
71 0.998639387560641
72 0.998639387560641
73 0.998639387560641
74 0.998639387560641
75 0.998639387560641
76 0.998639387560641
77 0.998639387560641
78 0.998639387560641
79 0.998639387560641
80 0.998639387560641
81 0.998639387560641
82 0.998639387560641
83 0.998639387560641
84 0.998639387560641
85 0.998639387560641
86 0.998639387560641
87 0.998639387560641
88 0.998639387560641
89 0.998639387560641
90 0.998639387560641
91 0.998639387560641
92 0.998639387560641
93 0.998639387560641
94 0.998639387560641
95 0.998639387560641
96 0.998639387560641
97 0.998639387560641
98 0.998639387560641
99 0.998639387560641
};
\addlegendentry{\(\policy_{base}\), Full Comm.}


\addplot [ultra thick, red, dashed]
table {%
0 0.82
1 0.82
2 0.82
3 0.82
4 0.82
5 0.82
6 0.82
7 0.82
8 0.82
9 0.82
10 0.82
11 0.82
12 0.82
13 0.82
14 0.82
15 0.82
16 0.82
17 0.82
18 0.82
19 0.82
20 0.82
21 0.82
22 0.82
23 0.82
24 0.82
25 0.82
26 0.82
27 0.82
28 0.82
29 0.82
30 0.82
31 0.82
32 0.82
33 0.82
34 0.82
35 0.82
36 0.82
37 0.82
38 0.82
39 0.82
40 0.82
41 0.82
42 0.82
43 0.82
44 0.82
45 0.82
46 0.82
47 0.82
48 0.82
49 0.82
50 0.82
51 0.82
52 0.82
53 0.82
54 0.82
55 0.82
56 0.82
57 0.82
58 0.82
59 0.82
60 0.82
61 0.82
62 0.82
63 0.82
64 0.82
65 0.82
66 0.82
67 0.82
68 0.82
69 0.82
70 0.82
71 0.82
72 0.82
73 0.82
74 0.82
75 0.82
76 0.82
77 0.82
78 0.82
79 0.82
80 0.82
81 0.82
82 0.82
83 0.82
84 0.82
85 0.82
86 0.82
87 0.82
88 0.82
89 0.82
90 0.82
91 0.82
92 0.82
93 0.82
94 0.82
95 0.82
96 0.82
97 0.82
98 0.82
99 0.82
};
\addlegendentry{\(\policy_{base}\), No Comm.}
% \end{axis}

% \end{tikzpicture}


==> tikz/success_prob_vs_iters_three_agent_aux_action.tex <==
% This file was created with tikzplotlib v0.9.12.
% \begin{tikzpicture}

% \begin{axis}[
% legend cell align={left},
% legend style={
%   fill opacity=0.8,
%   draw opacity=1,
%   text opacity=1,
%   at={(0.03,0.03)},
%   anchor=south west,
%   draw=white!80!black
% },
% tick align=outside,
% tick pos=left,
% title={Policy Success Probability During Synthesis},
% x grid style={white!69.0196078431373!black},
% xlabel={Number of Convex-Concave Iterations},
% xmajorgrids,
% xmin=-2.5, xmax=52.5,
% xtick style={color=black},
% y grid style={white!69.0196078431373!black},
% ylabel={Total Correlation Value},
% ymajorgrids,
% ymin=-1.0297070434498, ymax=1.08755937162852,
% ytick style={color=black}
% ]

\addplot [ultra thick, blue, mark=*, mark size=0, mark options={solid}]
table {%
0 0.0660480345962676
1 0.21287529321455
2 0.573625571177581
3 0.780548018736779
4 0.83452728129347
5 0.842791743430806
6 0.841688386047184
7 0.838843247077028
8 0.836011172463502
9 0.833930955296176
10 0.832807635009755
11 0.832453702149428
12 0.832524205013572
13 0.832749169563753
14 0.832992407080036
15 0.833206929078415
16 0.833396715155867
17 0.83367028244825
18 0.834663710841716
19 0.837888195182434
20 0.841527817502073
21 0.843669679129457
22 0.844810779821129
23 0.845447508953732
24 0.845851750364748
25 0.84603693435991
26 0.846056537900492
27 0.846011382925181
28 0.845949659754369
29 0.845904157886998
30 0.84590074387887
31 0.845964829530159
32 0.846088740910412
33 0.846214878359156
34 0.846302467730236
35 0.84635401913563
36 0.846383268076151
37 0.846399944056496
38 0.846409536162457
39 0.846415067191378
40 0.846418202502701
41 0.846419856467588
42 0.846420576340201
43 0.846420667772602
44 0.846420324415006
45 0.84641965746048
46 0.846418739167436
47 0.846417618026765
48 0.846416339735901
49 0.846414945253406
50 0.846413457062489
};
\addlegendentry{\(\policy_{MD}\), Full Comm.}

\addplot [ultra thick, blue, dashed]
table {%
0 0.012
1 0.081
2 0.176
3 0.302
4 0.306
5 0.344
6 0.281
7 0.285
8 0.269
9 0.274
10 0.215
11 0.267
12 0.251
13 0.255
14 0.247
15 0.285
16 0.264
17 0.283
18 0.348
19 0.598
20 0.689
21 0.691
22 0.683
23 0.701
24 0.705
25 0.714
26 0.68
27 0.705
28 0.719
29 0.711
30 0.716
31 0.705
32 0.691
33 0.692
34 0.682
35 0.697
36 0.709
37 0.688
38 0.701
39 0.705
40 0.674
41 0.683
42 0.696
43 0.687
44 0.707
45 0.682
46 0.689
47 0.69
48 0.697
49 0.725
50 0.697
};
\addlegendentry{\(\policy_{MD}\), No Comm.}

\addplot [ultra thick, red, mark=*, mark size=0, mark options={solid}]
table {%
0 0.991319989124963
1 0.991319989124963
2 0.991319989124963
3 0.991319989124963
4 0.991319989124963
5 0.991319989124963
6 0.991319989124963
7 0.991319989124963
8 0.991319989124963
9 0.991319989124963
10 0.991319989124963
11 0.991319989124963
12 0.991319989124963
13 0.991319989124963
14 0.991319989124963
15 0.991319989124963
16 0.991319989124963
17 0.991319989124963
18 0.991319989124963
19 0.991319989124963
20 0.991319989124963
21 0.991319989124963
22 0.991319989124963
23 0.991319989124963
24 0.991319989124963
25 0.991319989124963
26 0.991319989124963
27 0.991319989124963
28 0.991319989124963
29 0.991319989124963
30 0.991319989124963
31 0.991319989124963
32 0.991319989124963
33 0.991319989124963
34 0.991319989124963
35 0.991319989124963
36 0.991319989124963
37 0.991319989124963
38 0.991319989124963
39 0.991319989124963
40 0.991319989124963
41 0.991319989124963
42 0.991319989124963
43 0.991319989124963
44 0.991319989124963
45 0.991319989124963
46 0.991319989124963
47 0.991319989124963
48 0.991319989124963
49 0.991319989124963
50 0.991319989124963
};
\addlegendentry{\(\policy_{base}\), Full Comm.}


\addplot [ultra thick, red, dashed]
table {%
0 0.161
1 0.161
2 0.161
3 0.161
4 0.161
5 0.161
6 0.161
7 0.161
8 0.161
9 0.161
10 0.161
11 0.161
12 0.161
13 0.161
14 0.161
15 0.161
16 0.161
17 0.161
18 0.161
19 0.161
20 0.161
21 0.161
22 0.161
23 0.161
24 0.161
25 0.161
26 0.161
27 0.161
28 0.161
29 0.161
30 0.161
31 0.161
32 0.161
33 0.161
34 0.161
35 0.161
36 0.161
37 0.161
38 0.161
39 0.161
40 0.161
41 0.161
42 0.161
43 0.161
44 0.161
45 0.161
46 0.161
47 0.161
48 0.161
49 0.161
50 0.161
};
\addlegendentry{\(\policy_{base}\), No Comm.}

% \end{axis}

% \end{tikzpicture}


==> tikz/total_corr_vs_iters_aux_action.tex <==
% This file was created with tikzplotlib v0.9.12.
\begin{tikzpicture}

% \begin{axis}[
% tick align=outside,
% tick pos=left,
% title={Total Correlation During Policy Synthesis},
% x grid style={white!69.0196078431373!black},
% xlabel={Number of Convex-Concave Iterations},
% xmajorgrids,
% xmin=-4.95, xmax=103.95,
% xtick style={color=black},
% y grid style={white!69.0196078431373!black},
% ylabel={Total Correlation Value},
% ymajorgrids,
% ymin=2.3047037702847, ymax=5.28826171186816,
% ytick style={color=black}
% ]
\addplot [ultra thick, green!50!black, mark=*, mark size=0, mark options={solid}]
table {%
0 5.15264544179619
1 4.68317271807378
2 4.39171327144698
3 4.21395948515888
4 4.11560745278937
5 4.06649668937908
6 4.03827022931464
7 4.01201823707948
8 3.9803339387189
9 3.94127240699369
10 3.89060171704013
11 3.81549846191682
12 3.69155241505934
13 3.49559290135641
14 3.25223716043656
15 3.04762402864481
16 2.92664609938956
17 2.8626372885865
18 2.8251925550615
19 2.79879422909851
20 2.7773058925953
21 2.75854620794905
22 2.741714437737
23 2.7264901335079
24 2.71258755580526
25 2.69977396710103
26 2.68789621688871
27 2.6768838231776
28 2.66666227426287
29 2.65710889221536
30 2.64809665171394
31 2.63950826708494
32 2.6312309785254
33 2.62315260567095
34 2.61516065145018
35 2.60714418811698
36 2.59899698434797
37 2.59062416556893
38 2.58195222772684
39 2.57294109395158
40 2.56359913830999
41 2.55399671613158
42 2.54427286041482
43 2.5346286325025
44 2.52530362043296
45 2.51653757569382
46 2.50852766766309
47 2.50139630039307
48 2.49518132325336
49 2.48984508893192
50 2.48529912823347
51 2.48142269446734
52 2.47808360722807
53 2.47519270456921
54 2.47274490330995
55 2.47066475651466
56 2.46886252648517
57 2.46728234756773
58 2.46588459521591
59 2.46464002594758
60 2.46352758801409
61 2.46252833440585
62 2.46162777482718
63 2.46081348036854
64 2.46007484857881
65 2.45940215991232
66 2.45878761319396
67 2.45822323800726
68 2.45770235155538
69 2.45721850221365
70 2.45676614015582
71 2.45633974276869
72 2.45593529515354
73 2.45554829838795
74 2.45517424498923
75 2.45480999376444
76 2.45445194684321
77 2.45409649569344
78 2.45374016581652
79 2.45338029431738
80 2.45301362638588
81 2.45263671350312
82 2.45224628537454
83 2.45183955766764
84 2.45141287605475
85 2.45096275000469
86 2.45048589330188
87 2.44997822588487
88 2.44943663998259
89 2.44885721972514
90 2.44823604585716
91 2.44757036480281
92 2.44685604586845
93 2.44609026070399
94 2.4452703634753
95 2.44439431366251
96 2.44346101218426
97 2.44246997378609
98 2.44142229820225
99 2.44032004035668
};
% \end{axis}

\end{tikzpicture}


==> tikz/total_corr_vs_iters_three_agent_aux_action.tex <==
% This file was created with tikzplotlib v0.9.12.
% \begin{tikzpicture}

% \begin{axis}[
% tick align=outside,
% tick pos=left,
% title={Total Correlation During Policy Synthesis},
% x grid style={white!69.0196078431373!black},
% xlabel={Number of Convex-Concave Iterations},
% xmajorgrids,
% xmin=-2.5, xmax=52.5,
% xtick style={color=black},
% y grid style={white!69.0196078431373!black},
% ylabel={Total Correlation Value},
% ymajorgrids,
% ymin=3.24403675317078, ymax=7.11588490332945,
% ytick style={color=black}
% ]
\addplot [ultra thick, green!50!black, mark=*, mark size=0, mark options={solid}]
table {%
0 6.93989180559497
1 6.0910933127967
2 6.35385494622104
3 6.2047257230844
4 5.78548343133209
5 5.48272543111571
6 5.28588562420308
7 5.14072186715017
8 5.02264300503871
9 4.93040566526548
10 4.86885793926025
11 4.83607455844947
12 4.82244314968019
13 4.81829544086787
14 4.81781152801878
15 4.81778962895869
16 4.81278838696478
17 4.77152950038468
18 4.52091782564644
19 3.83629538589137
20 3.52841131518657
21 3.47889903438276
22 3.45041673463197
23 3.43872675105157
24 3.43257323923111
25 3.4285396029474
26 3.42553470514334
27 3.42325338910333
28 3.42165287150888
29 3.42058877434084
30 3.42002985090527
31 3.42004994248731
32 3.4205660113963
33 3.42116550124794
34 3.4215539102942
35 3.42174624468508
36 3.42182932359968
37 3.42185712910935
38 3.42185642604074
39 3.4218399490861
40 3.42181409358213
41 3.42178225763336
42 3.42174599875438
43 3.42170640449942
44 3.42166392615828
45 3.42161906238366
46 3.42157198035698
47 3.42152287062943
48 3.42147216452707
49 3.42142012674573
50 3.42136748561844
};
% \end{axis}

% \end{tikzpicture}

